On the control of the load increments for a proper description of multiple delamination in a domain decomposition framework

In quasi-static nonlinear time-dependent analysis, the choice of the time discretization is a complex issue. The most basic strategy consists in determining a value of the load increment that ensures the convergence of the solution with respect to time on the base of preliminary simulations. In more advanced applications, the load increments can be controlled for instance by prescribing the number of iterations of the nonlinear resolution procedure, or by using an arc-length algorithm. These techniques usually introduce a parameter whose correct value is not easy to obtain. In this paper, an alternative procedure is proposed. It is based on the continuous control of the residual of the reference problem over time, whose measure is easy to interpret. This idea is applied in the framework of a multiscale domain decomposition strategy in order to perform 3D delamination analysis.

==> notations.tex <==
%--------------- trucs a moi -----------------------------
%commandes PK
\newcommand{ \V }[1]{ \underline{#1} }
\newcommand{ \M }[1]{ \underline{\underline{#1}} }
\RequirePackage{amsmath,amssymb,bm}% …tendre les fonctions maths
\usepackage[ruled,section]{algorithm}
\usepackage{algorithmic,url,rotating}
\usepackage{subfigure}
\usepackage{stmaryrd}

\newcommand{\ply}{{P}}
\newcommand{\plyprime}{{P'}}
\newcommand{\domainply}{{\Omega_P}}
\newcommand{\domainplyprime}{{\Omega_{P'}}}
\newcommand{\uply}{{\underline{u}_P}}
\newcommand{\sigply}{{\underline{\underline{\sigma}}_P}}
\newcommand{\epsply}{{\underline{\underline{\epsilon}}_P}}
\newcommand{\interply}{{I_{PP'}}}
\newcommand{\prescrforce}{{\underline{F}_d}}
\newcommand{\prescrdep}{{\underline{U}_d}}
\newcommand{\voluforce}{{\underline{f}_d}}
\newcommand{\normalply}{{\underline{n}_p}}
%domaine
\newcommand{\domain}{{\Omega}}
\newcommand{\struct}{{\mathbf{E}}}
\newcommand{\dOmega}{{\partial \Omega}}
\newcommand{\dOmegau}{{\partial \Omega_u}}
\newcommand{\dOmegaf}{{\partial \Omega_f}}
\newcommand{\Fd}{{\underline{F}_d}}
\newcommand{\Ud}{{\underline{U}_d}}
\newcommand{\fd}{{\underline{f}_d}}
%sous-structuration
\newcommand{\substruct}{{E}} % en double
\newcommand{\E}{{E}}
\newcommand{\VE}{{\mathbf{V}_E}}
\newcommand{\Esub}{{\mathbf{E_{\textrm{sub}}}}}
\newcommand{\Ep}{{E'}}
\newcommand{\subdomain}{{\Omega_E}} % en double
\newcommand{\OmegaE}{{\Omega_E}}
\newcommand{\OmegaEp}{{\Omega_{E'}}}
\newcommand{\Omegasub}{{\Omega_{\textrm{sub}}}}
\newcommand{\dOmegasub}{{\partial \Omega_{\textrm{sub}}}}
\newcommand{\bordsubdomain}{{\partial \Omega_E}} % en double
\newcommand{\dOmegaE}{{\partial \Omega_E}}
\newcommand{\compsubstruct}{{\mathbf{\bar{E}}} }% en double
\newcommand{\Ebar}{{\bar{E}}}
\newcommand{\GammaEEp}{{\Gamma_{EE'}}}
\newcommand{\GammaE}{{\Gamma_E}}
\newcommand{\GammaEd}{{\Gamma_{{E}_d}}}
\newcommand{\supE}{{\bar{E}}}
\newcommand{\supEp}{{\bar{E'}}}
\newcommand{\OmegasupE}{{\Omega_{\bar{E}}}}
\newcommand{\supGammaEEp}{{\Gamma_{\bar{E}\bar{E'}}}}
\newcommand{\dOmegasupE}{{\partial \Omega_{\bar{E}}}}
%variables sst
\newcommand{\uE}{{\underline{u}_E}}
\newcommand{\uEstar}{{\underline{u}_E}^{\star}}
\newcommand{\epsilonE}{{\underline{\underline{\epsilon}}(\underline{u}_E)}}
\newcommand{\sigmaE}{{\underline{\underline{\sigma}}_E}}
\newcommand{\epsilonEstar}{{\underline{\underline{\epsilon}}({\underline{u}_E}^{\star})}}
\newcommand{\KE}{{\mathbf{K}}}
\newcommand{\FE}{{\underline{F}_E}}
\newcommand{\FmE}{{\underline{F}_E^m}}
\newcommand{\FME}{{\underline{F}_E^M}}
\newcommand{\WE}{{\underline{W}_E}}
\newcommand{\WEstar}{{{\underline{W}_E}^{\star}}}
\newcommand{\WMEstar}{{{\underline{W}_E^M}^{\star}}}
\newcommand{\WmE}{{\underline{W}_E^m}}
\newcommand{\WME}{{\underline{W}_E^M}}
\newcommand{\WtildeE}{{\underline{\widetilde{W}}_E^M}}
\newcommand{\WtildeEstar}{{\underline{\widetilde{W}}_E^M}^{\star}}
\newcommand{\kmE}{{k^-_E}}
\newcommand{\hmE}{{h^-_E}}
\newcommand{\kpE}{{k^+_E}}
\newcommand{\kpEEp}{{k^+_{EE'}}}
\newcommand{\kpEp}{{k^+_{E'}}}
\newcommand{\kmME}{{{k_E^-}^M}}
\newcommand{\kpME}{{{k_E^+}^M}}
\newcommand{\kmmE}{{{k_E^-}^m}}
\newcommand{\kpmE}{{{k_E^+}^m}}
\newcommand{\kmmEEp}{{{k_{EE'}^{-^m}}}}
\newcommand{\kmEEp}{{k_{EE'}^{-}}}
\newcommand{\kmMEEp}{{{k_{EE'}^{-^M}}}}
\newcommand{\FchapchapE}{{\underline{\widehat{\widehat{F}}}_E}}
\newcommand{\FchapE}{{\underline{\widehat{F}}_E}}
\newcommand{\WchapE}{{\underline{\widehat{W}}_E}}
\newcommand{\FchapME}{{\underline{\widehat{F}}_E^M}}
\newcommand{\WchapME}{{\underline{\widehat{W}}_E^M}}
\newcommand{\FchapMEp}{{\underline{\widehat{F}}_{E'}^M}}
\newcommand{\WchapMEp}{{\underline{\widehat{W}}_{E'}^M}}
%variables interfaces
\newcommand{\FchapEp}{{\underline{\widehat{F}}_{E'}}}
\newcommand{\WchapEp}{{\underline{\widehat{W}}_{E'}}}
\newcommand{\FEp}{{\underline{F}_{E'}}}
\newcommand{\WEp}{{\underline{W}_{E'}}}
\newcommand{\FMEp}{{\underline{F}_{E'}^M}}
\newcommand{\WMEp}{{\underline{W}_{E'}^M}}
\newcommand{\Wtilde}{{\underline{\widetilde{W}}^M}}
\newcommand{\Wtildestar}{{{\underline{\widetilde{W}}^M}^{\star}}}
\newcommand{\kmMEp}{{{{k_{E'}^-}^M}}}
\newcommand{\kpMEp}{{{{k_{E'}^+}^M}}}
\newcommand{\kmmEp}{{{{k_{E'}^-}^m}}}
\newcommand{\kpmEp}{{{{k_{E'}^+}^m}}}
\newcommand{\kmnE}{{{k_n}^-_E}}
\newcommand{\kmtE}{{{k_t}^-_E}}
\newcommand{\kECL}{{k_E^{\textrm{CL}}}}
\newcommand{\FECL}{{\underline{F}_E^{\textrm{CL}}}}
\newcommand{\WECL}{{\underline{W}_E^{\textrm{CL}}}}
\newcommand{\sautWE}{{\underline{[W]}_E}}
\newcommand{\sautWmE}{{\underline{[W]}_E^m}}
\newcommand{\sautWME}{{\underline{[W]}_E^M}}
\newcommand{\F}{{\underline{F}}}
\newcommand{\W}{{\underline{W}}}
\newcommand{\Wstar}{{\underline{W}^{\star}}}
\newcommand{\FM}{{\underline{F}^M}}
\newcommand{\WM}{{\underline{W}^M}}
\newcommand{\WMstar}{{\underline{W}^{M^{\star}}}}
\newcommand{\Fm}{{\underline{F}^m}}
\newcommand{\Wm}{{\underline{W}^m}}
\newcommand{\PiMEEp}{{{\boldsymbol{\Pi}}_{EE'}^M}}

%variables sst voisine

%espaces
\newcommand{\sWE}{{\mathcal{W}_E}}
\newcommand{\sWEO}{{\mathcal{W}_E^0}}
\newcommand{\sWmE}{{\mathcal{W}_E^m}}
\newcommand{\sWME}{{\mathcal{W}_E^M}}
\newcommand{\sWMEO}{{\mathcal{W}_E^{M^0}}}
\newcommand{\sFE}{{\mathcal{F}_E}}
\newcommand{\sFmE}{{\mathcal{F}_E^m}}
\newcommand{\sFME}{{\mathcal{F}_E^M}}
\newcommand{\sAd}{\mathbf{A_d}}
\newcommand{\sGamma}{{\boldsymbol{\Gamma}}}
\newcommand{\suE}{{\mathcal{U}_E}}
\newcommand{\suEO}{{\mathcal{U}_E^0}}
\newcommand{\ssigmaE}{{\mathcal{S}_E}}
\newcommand{\suEh}{{\mathcal{U}_E^h}}
\newcommand{\sWEh}{{\mathcal{W}_E^h}}
\newcommand{\sFEh}{{\mathcal{F}_E^h}}
\newcommand{\sF}{{\mathcal{F}}}
\newcommand{\sW}{{\mathcal{W}}}
\newcommand{\sFM}{{\mathcal{F}^M}}
\newcommand{\sWM}{{\mathcal{W}^M}}
\newcommand{\sFm}{{\mathcal{F}^m}}
\newcommand{\sWm}{{\mathcal{W}^m}}
\newcommand{\sFEEp}{{\mathcal{F}_{EE'}}}
\newcommand{\sWEEp}{{\mathcal{W}_{EE'}}}
\newcommand{\sFMEEp}{{\mathcal{F}^M_{EE'}}}
\newcommand{\sWMEEp}{{\mathcal{W}^M_{EE'}}}
\newcommand{\sFmEEp}{{\mathcal{F}^m_{EE'}}}
\newcommand{\sWmEEp}{{\mathcal{W}^m_{EE'}}}
\newcommand{\sEp}{{\mathbf{E^+}}}
\newcommand{\sEm}{{\mathbf{E^-}}}
\newcommand{\sWMad}{{\mathcal{W}^M_\textrm{ad}}}
\newcommand{\sFMad}{{\mathcal{F}^M_\textrm{ad}}}
\newcommand{\sWMsupad}{{\bar{\mathcal{W}}^M_\textrm{ad}}}


%autres
\newcommand{\dvol}{d \Omega}
\newcommand{\dsurf}{d \Gamma}
\newcommand{\Rd}{\mathcal{R}_d}
\newcommand{\R}{\mathcal{R}}

%commandes PG
\newcommand{\Ks}{\ensuremath{\mathcal{K}}}
\newcommand{\Ls}{\ensuremath{\mathcal{L}}}
\newcommand{\Cs}{\ensuremath{\mathcal{C}}}
\newcommand{\iden}{\ensuremath{\mathbf{I}}}
\newcommand{\op}{\ensuremath{\mathbf{A}}}
\newcommand{\pppreco}{\ensuremath{\tilde{\op}}}
\newcommand{\preco}{\ensuremath{\tilde{\op}^{-1}}}
\newcommand{\precoT}{\ensuremath{\tilde{\op}^{-T}}}
\newcommand{\const}{\ensuremath{C}}
\newcommand{\proj}{\ensuremath{\mathbf{P}}}

%--------------- fin trucs a moi -----------------------------x
